Large Language Models Struggle to Describe the Haystack without Human Help: Human-in-the-loop Evaluation of Topic Models

A common use of NLP is to facilitate the understanding of large document collections, with a shift from using traditional topic models to Large Language Models. Yet the effectiveness of using LLM for large corpus understanding in real-world applications remains under-explored. This study measures the knowledge users acquire with unsupervised, supervised LLM-based exploratory approaches or traditional topic models on two datasets. While LLM-based methods generate more human-readable topics and show higher average win probabilities than traditional models for data exploration, they produce overly generic topics for domain-specific datasets that do not easily allow users to learn much about the documents. Adding human supervision to the LLM generation process improves data exploration by mitigating hallucination and over-genericity but requires greater human effort. In contrast, traditional. models like Latent Dirichlet Allocation (LDA) remain effective for exploration but are less user-friendly. We show that LLMs struggle to describe the haystack of large corpora without human help, particularly domain-specific data, and face scaling and hallucination limitations due to context length constraints.

==> scripts/style-check/bad-words <==
utilize              % phrase "use" http://www.bartleby.com/64/C003/0294.html
utilizes             % phrase "uses" http://www.bartleby.com/64/C003/0294.html
utilized             % phrase "used" http://www.bartleby.com/64/C003/0294.html
utilizing            % phrase "using" http://www.bartleby.com/64/C003/0294.html
leverage             % phrase "use"
abstraction          % phrase this is often used poorly?
fashion              % phrase hrm.
[dw]on't             % spelling do not or will not.
behavioral           % spelling I'm convinced we don't use this word properly.
we'll                % spelling we will
we've                % spelling we have
[^r][^c][^h] impact  % phrase "consequences", "effect", "result", though nsf likes "research impact"
tackle               % phrase "tackle" (a problem) is wimpy for "solve" or a tired metaphor for "address a challenge".
thusly               % phrase "thus" or "this way" or "like this" http://www.bartleby.com/64/C003/0282.html
transpire            % phrase "happen" 
so-called            % phrase can be abused; it's negative.
necessitate          % phrase require.
necessitated         % phrase required.
necessitates         % phrase requires.
loosing              % spelling you almost certainly mean "losing".  use "loosening" otherwise.
aforementioned       % phrase too pretentious.
important to         % phrase "valued by"?
notion               % phrase avoid this weak phrase. (thanks brian bershad!)
achieve(s)?\s        % phrase models don't achieve anything, only use for humans
reasonably           % phrase hedging


==> scripts/style-check/common-typos <==
a the                % phrase double article
 pt                  % syntax ? I guess avoid straggling pt's that escape tex?
[ ],                 % syntax whitespace before comma seems wrong.
Figure Figure        % phrase pizza pizza.
[ ]-[ ]              % syntax a hyphen surrounded by space should probably be an emdash '---'
[0-9]-[0-9]          % syntax use an endash '--' for ranges
[0-9]ms              % syntax put a space between the number and the unit.
[^egs]\. [a-z]       % syntax a period usually ends a sentence, and sentences should start with a capital; doesn't apply for i.e.,
\.  [a-z]            % syntax a period usually ends a sentence, and sentences should start with a capital; "i.e." should have a comma following.
[a-z]\.\.            % syntax double period is rarely right, use \ldots for ellipsis
[^\\]"               % syntax use fancy quotes
\beg\.               % syntax should be e.g. as in "examples given"
from to\b            % phrase haven't used this properly.
help help            % phrase double word, that probably means the author paniced
of of                % phrase apparent double word.
the affect           % phrase should probably be 'the effect'
the the              % phrase apparent double word.
there too few        % phrase there are too few?
was not was          % phrase pretty much a joke if this gets matched.
we we                % phrase it would be oi oi in french, I guess.
with on              % phrase probably wrong.
with with            % phrase apparent double word.
[\n ]--[\n ]         % syntax that's an en-dash, you want an em-dash: "---"
my my                % phrase unlikely that's what you want, at least without a comma. (doesn't work across newlines)
>From                % syntax be careful when you email .tex files.  I've seen this slip through into submissions.
e\.t\.c\.            % syntax it's et cetera; use etc.
such as like         % phrase pick one
<<<<<<< .            % syntax CVS conflict!
=======              % syntax CVS conflict!
>>>>>>> [0-9]        % syntax CVS conflict!
e\.g\.[\n ]          % syntax should be followed with a comma, as e.g. can be read as "for example" (thanks JZ!)
i\.e\.[\n ]          % syntax should be followed with a comma, as i.e. can be read as "that is" (thanks JZ!)
[ ]\.[\n ]           % syntax stray period?
further more         % phrase one word: furthermore
safe guard           % phrase one word: safeguard
that be              % phrase mistake.
can not              % phrase cannot
only only            % phrase double word
is is                % phrase double word.
they shows           % phrase argh, mistake.
less that than       % phrase typo damage
from from            % phrase double word score
in in                % phrase "in" (common mistake)
not not              % phrase argh.
it it                % phrase argh.
to illicit           % phrase "to elicit" -- illicit is always an adjective.
c\.f\.               % phrase actually, it's cf., and you'd like cf.\ (backslash space)
this lead to         % phrase "led to" if past tense, "leads to" if present.
on on                % phrase double word.
has is               % phrase choose
description their    % phrase saw this, clearly wrong.
including:  % syntax I prefer no colon after including, which already says a list is coming.
[a-z]\([A-Z]  % syntax put a space before parens, even when introducing acronyms.
without and without % phrase saw this.
can be result       % phrase saw this typo.



==> scripts/style-check/foolish-phrases <==
(quite|more|very|most) unique    % phrase unique is.
(quite|more|very|most) abstract  % phrase abstract is.
tangible view                    % phrase mix that metaphor some more.
for e\.g\.                       % phrase e.g. includes "for".
begs the question                % phrase unless you're very clever: "raises the question": http://alt-usage-english.org/excerpts/fxbegthe.html
high rate of speed               % phrase local news-speak.
especially necessary             % phrase 'especially important', necessary may be an absolute like unique.
how will it effect % phrase you likely meant "affect"
how it will effect % phrase you likely meant "affect"
insure proper performance % phrase "ensure"
especially true                  % phrase 'especially important', true may be an absolute like unique.
to affect change                 % phrase "effect" change;  I read this on a poster.
higher results                   % phrase maybe higher performance or higher values.
is more general then the         % phrase probably "than"
upper bounding                   % phrase "limiting" or "setting an upper bound on"
in principal                     % phrase likely, "in principle"
literally like                   % phrase literally means no simile.  
design principal  % phrase likely, "design principle" 
different from 	    	   	 % phrase unlike

==> scripts/style-check/latex-checking <==
\{\\em [^\}]*[^\}\/]\}[:]    % syntax use \emph{} or explicit italic correction {\em foo\/}
\{\\em [^\}]*[:\.,]\}        % syntax punctuation at the edges of italic text is not italicized
[A-Z]{2,10}\.[ ]*[\n ][ ]*[A-Z]  % syntax intersentence spacing should be used if a sentence ends with an acronym: "FOO\\@."
\\etal[^{]                   % syntax it's good practice to use \etal{} to avoid bad spacing
\\caption\[[^\]]*[^\.]\]     % syntax short caption should end with a period.
\\caption\[.*CCDF.*\]        % syntax short caption should not include graph type.
\\caption\[.*CDF.*\]         % syntax short caption should not include graph type.
\\caption\[.{0,25}\]         % syntax short caption should not be too short.
th century                   % syntax use textsuperscript
[ ]---[ ]                    % syntax the em-dash should be right up against the words.
[ \n]---[ \n]                % syntax the em-dash should be right up against the words.
^---[ \n]                    % syntax the em-dash should be right up against the words.
[ \n]---$                    % syntax the em-dash should be right up against the words.
[ \n]--[ \n]                 % syntax the en-dash should be between numbers.
^--[ \n]                     % syntax the en-dash should be between numbers.
[ \n]--$                     % syntax the en-dash should be rbetween numbers.
,[~ ]\\etal                  % syntax no comma before etal (unless Smith, Martinez, \etal)
\\etal\{\}'s                 % syntax eew.
\\(sub)?section\{[A-Z][^}]*[ ][a-z]{5,40}[^}]*\} % syntax subsection headers should be initial capped.
\\(sub)?section\{[A-Z][^}]*[^:][ ]{1,}(With|A|An|Is|And|For|To|The)[ ][^}]*\} % syntax some words needn't be capitalized
[ ]\\footnote                % syntax no space before footnote.
\\footnote\{.*\}.            % syntax footnotes after punctuation
,,                           % syntax double comma is unlikely to be intentional.
cf\.[^\\]                    % phrase cf. should get an escaped space "\ "
et al\.[^\\]                    % phrase et al. should get an escaped space "\ "
[<>]  % syntax a less than or greater than outside math mode shows other characters.
in (section|table|figure) \\ref % phrase should have ~ before ref
section~\\ref % capitalize capitalize section when saying Section 6.
table~\\ref % capitalize capitalize section when saying Table 6.
figure~\\ref % capitalize capitalize section when saying Figure 6.
\\(sub)?section\{Intro\} % syntax spell it out.
,''                          % syntax punctuation outside quotes
\.\.\.                       % syntax use \dots

==> scripts/style-check/my-rules <==
#  such may be abused to blacklist certain words even spelled correctly.
# capitalize is case sensitive, and also bracketed by non-word.
# phrase and spelling are case insensitive, but bracketed by non-word characters.
# syntax is case sensitive but not bracketed by non-word; probably best if used with regexes.
\bet al\.[^}]        % syntax use the \etal{} command instead. (or write one to italicize)
\bet\. al\.          % syntax use the \etal{} command, "et" needs no dot (et alii). (or write one to italicize)
\bc\.f\.\b             % syntax should be cf. for "confer" (latin for compare)
\b$i\)[^$]              % syntax leave the paren in math mode -- should be $i)$
\b$ii\)[^$]             % syntax leave the paren in math mode -- should be $ii)$
\b$iii\)[^$]            % syntax leave the paren in math mode -- should be $iii)$
\b$iv\)[^$]             % syntax leave the paren in math mode -- should be $iv)$
\b$v\)[^$]              % syntax leave the paren in math mode -- should be $v)$
\ban [b-df-gj-np-tv-z] % syntax probably meant to use "a" instead of "an", though there are exceptions.
\ban [B-DF-GJ-NP-TV-Z][^A-Z/] % syntax probably meant to use "a" instead of "an", though there are exceptions (like acronyms).
\b[Aa] [aeiouAEIOU](?!se|ni|A|ur|RL|ti|ne|DP) % syntax probably meant to use "an" instead of "a", though there are exceptions. (user, useful, AA, unified, uniform, unique, Europe, one, UDP; n/a doesn't work, so use {n/a})
This allows           % phrase tie more explicitly: This (x) allows...
we find               % phrase omit "we find"
we found              % phrase omit "we found"
try and               % phrase "try to", though if you're using try as a noun in a compound sentence, this rule is wrong.
impact of             % phrase not a useful metaphor; try evaluation, success, effect, value.
including [^\.]*etc\. % syntax "including" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
includes [^\.]*etc\.  % syntax "includes" tells of a non-exclusive list, so "etc." is redundant.  This rule will misfire if you have two lists in your sentence, but you shouldn't do that either. ;)
and etc\.             % phrase come on. learn some latin.
AT&T                  % syntax you poor thing, this won't compile.
doesn't               % phrase be formal.
be occur              % phrase what happens when I'm indecisive about what follows "can"
up until              % phrase "until"
one or more           % phrase probably redundant -- nonzero is probably implied.
is comprise(d|s) of   % phrase you probably mean "is composed of" because "comprises" is more a synonym for "contains" 
will be significantly different % phrase "will differ significantly" for active voice
More importantly,     % phrase probably means the order is wrong: put important stuff first.
todo                  % ignoredcommand
texttt                  % ignoredcommand
jbgcomment              % ignoredcommand
lkfcomment              % ignoredcommand
due to space constraints % phrase don't whine.
this paper % phrase can be ambiguous if talking about someone else's paper whether you mean the one youre writing or the one you're talking about..
the above             % phrase horrible phrase that must be expunged.  you might use "these" instead, but best to make the sentence stand alone.
referred to above     % phrase "these".
(all|the|of) [0-9][ ] %  phrase use words for numbers in phrases.
clearly shows         % phrase "clearly" is usually much.
grows larger          % phrase is "grows smaller" possible?  grows.
guarantee as much as possible % phrase then not really a guarantee "provide"
affects negatively   % phrase "hurts" or "harms"
rely upon % phrase rely on is good enough
relies upon % phrase relies on is good enough
record route packets? % phrase hyphenate record-route packets
record-route; % phrase leave record route alone if not modifying something else
we accomplish this  % phrase verbose way to get active voice.
refers to the % phrase you're being wimpy in the definition.  use "is"
\\emph\{[a-zA-Z ]*\} refers to % syntax you're being wimpy in the definition.
loss off % phrase loss of?
this could % phrase this "what" could
with that has % phrase probably just one
simply % phrase probably isn't.
to get to % phrase "to reach"?
latency benefit % phrase reduction
latency improvement % phrase reduction
shed insight % phrase 'shed light' would seem the metaphor.
increasingly more % phrase redundant
I\.e\. % syntax starting a sentence with i.e. is just ugly.
E\.g\. % syntax starting a sentence with e.g. is just ugly.
in the large % phrase if large is a noun, bad.  if it's an adjective, fine.
encapsulates with % phrase seen it, don't know what it means.
when working with % phrase just say "with"
it is true that	  % phrase usually can delete
LDA % phrase convention put in small caps
(F|f)indings (show|indicate|suggest)	% phrase delete or make more specific

==> scripts/style-check/networking-research <==
IPs                  % phrase should be IP addresses
[Rr]ate-limits       % spelling "rate limits" has no hyphen, only "rate-limited"
best effort          % phrase hyphenate best-effort service.
deliver route        % phrase jargon redundancy
euclidean % capitalize Euclidean.
interdomain          % spelling inter-domain
internet             % capitalize unless talking about an internet other than the Internet
intradomain          % spelling intra-domain
log-normal           % spelling lognormal is one word.
pareto               % capitalize
ttl                  % capitalize
weibull              % capitalize proper name.
PoP                  % syntax I think POP looks less annoying.
PoPs                 % syntax I think POP looks less annoying.
http[ ]              % capitalize capitalize HTTP.
linux                % capitalize capitalize Linux
Internet[^\.]*Internet % syntax avoid Internet twice in the same sentence?
zipf                 % capitalize capitalize the guy's name.


==> scripts/style-check/passive-voice <==
it is possible to                   % phrase passive voice, try: "can"
are identified by                   % phrase passive
is shown                            % phrase passive.
is not included in                  % phrase maybe this is passive
there (are|is) [^\.:;]* (that|in)   % phrase maybe this is passive
can be evaluated                    % phrase avoid passive: I evaluated
can be observed                     % phrase avoid passive: are visible
# is needed                         % phrase passive voice
is used to                          % phrase go active voice, or subsititute "helps"
(are|were) needed[^\?]              % phrase passive voice
(is|are) presented in               % phrase "appears in", or reword to avoid passive voice
it is possible that                 % phrase "may"
(is|are) (depicted|illustrated|sketched) in  % phrase thats passive voice
(is|are) shown in                   % phrase "shows"
as can be seen in                   % phrase X shows that Y.
there needs to be                   % phrase passive voice in a bad way.
was designed                        % phrase passive voce.
it may be                           % phrase passive "it"
it is important that                % phrase passive; replace with X is important because Y.


==> scripts/style-check/verbose-phrases <==
a large number of                   % phrase you mean "many"
a substantial number of             % phrase how substantial?  most?  or just enough that can't be ignored?
an insufficient number of           % phrase "too few"
a significant number of             % phrase one is significant.   consider "prohibitive" if the number is sufficient to be problematic.
a number of                         % phrase getting the verb agreement for this useless phrase is tricky.
a number of different               % phrase use "different" (should have a high score)
a small number of                   % phrase you mean "few"
a low number of                   % phrase you mean "few"
a relatively low number of                   % phrase you mean "few"
actually                            % spelling probably doesn't add
to an extent                        % phrase you can probably remove
and instead                         % phrase replace with but?
be done                             % phrase if "X of Y can be done", try "Y can be Xed"; it's already passive voice.
combining multiple                  % phrase as opposed to "combining one?"
aggregating multiple                % phrase "aggregating"
do this                             % phrase probably verbose if you use a pronoun for what you're doing
exists[ ]                           % phrase probably no better than "is", but end of sentence may be unavoidable?
if it is to                         % phrase should be "to" (usually followed by "be X")
if they are to                      % phrase should be "to" (usually followed by "be X")
in general                          % phrase unless matched with "in specific," this is usually useless; perhaps "overall"
in order to                         % phrase remove "in order" and get "to"
in the past                         % phrase past tense is likely enough.
in the way of                       % phrase should be "as"
counting the number of              % phrase counting.  dude.
is permitted to                     % phrase "may"
largely opaque                      % phrase largely does not modify opaque
makes a new                         % phrase should be "creates"
may not chose                       % phrase "may not" is future tense; "chose" is past.
one should note                     % phrase just write it.
note that                           % phrase is the rest of the paper less notable?
Note, that                          % syntax not only should you not "note that", no comma after note.
we note                             % phrase is the rest of the paper less notable?
note however that                   % phrase is the rest of the paper less notable?
it is important to note             % phrase is the rest of the paper less notable?
really                              % phrase probably doesn't add; if you think it does, use "r{}eally" -- don't change to 'in fact'
in fact				    % phrase cut
rigorously                          % spelling probably doesn't add, and I rarely do anything with rigor
the way in which                    % phrase should be "how" or ""
the manner in which                 % phrase should be "how" or ""
value stems                         % phrase value is derived or offered, I think.
time at which                       % phrase very likely "when"
place at which                      % phrase very likely "where"
at the time                         % phrase very likely "when"
reduced number of                   % phrase very likely "fewer" or maybe maybe "less"
is present in                       % phrase present is probably redudant, try "is in"
they all                            % phrase maybe "all xs" would be better.
easy to do                          % phrase "feasible" or "practical" might be better.
is going to                         % phrase "will".
are going to                        % phrase "will".
getting                             % phrase probably "receiving" or "querying"
those are                           % phrase see if "those X are" is clearer?
design is motivated                 % phrase "inspired by" is probably better than "motivated" for design
locations throughout the world      % phrase drop "throughout the world"
e.g., as opposed to                 % phrase if you're giving examples, you're not talking about what isn't.  drop "e.g."
in addition, we also                % phrase remove either "also" or "in addition"
other related issues                % phrase probably remove "other"
the aforementioned                  % phrase "these xs" or "this x" would be less snooty
center around                       % phrase (cook) a center is a point: "center on" is okay.
could care less                     % phrase (cook) 'really? how much less could you care?' (should be couldn't)
grouped together                    % phrase redundant.  "grouped" alone should suffice.
put together                        % phrase long: "construct" "build" or "assemble"
consistent with each other          % phrase redundant.  "consistent" suffices.
be accomplished with                % phrase try "requires" "uses" "needs"?
the lack of knowledge of            % phrase would "X is unknown" work better?
gets to know                        % phrase you mean "learns"
trying to look like                 % phrase you mean "acting", "emulating", or "mimicing"
has got to be                       % phrase "must be"
got                                 % phrase try "became" "received" ?
gotten                              % phrase try "helped" ?
live in a vacuum                    % phrase a tired metaphor that makes me want to vomit.
positive impact                     % phrase try "benefit"
negative impact                     % phrase try "harm" or "consequences"
adverse impact                      % phrase try "harm" or "consequences"
adversely impacting                 % phrase try "harming" or "hurting"
discuss the issues of               % phrase could probably drop "the issues of" unless there's a list
the presence of                     % phrase not far from 'is', 'has', etc.
does not allow                      % phrase consider "forbids" or "prohibits"
and/or                              % phrase just say or.
there is the potential to           % phrase just say may.
there is the possibility that       % phrase just say might.
can be achieved                     % phrase maybe not so good?
find out                            % phrase perhaps determine?
in the absence of                   % phrase perhaps without?
in the presence of                  % phrase perhaps with?
set up                              % phrase perhaps create, configure, or initialize
in the face of                      % phrase can be overused.  try despite?
several times (at|of)               % phrase discouraged by Kurt.
a large degree of                   % phrase ick.
we start by first                   % phrase redundant. ("first, we" or "we start by").
in general, they are usually        % phrase redundant.
refers to the notion                % phrase define your term precisely if possible.
a significant amount of             % phrase probably just "significant"
real practical                      % phrase as opposed to imaginary practical?
people that are                     % phrase use people who are?
additional detail that we add       % phrase as opposed to additional detail that we subtract?
in some cases and not in others     % phrase "in some cases"
it is known that                    % phrase just say it.
caused due to                       % phrase "caused by"
a result of the fact that           % phrase "caused by"
results (indicate|show|suggest)     % phrase drop
research (indicates|show|suggest)   % phrase drop
can be attributed to the fact that  % phrase "is because"
a large set of                      % phrase probably don't care that it is a set.
a small set of                      % phrase probably don't care that it is a set: use 'a few'
provides a look at                  % phrase (timid) probably mean "shows".
in most cases                       % phrase "usually"
continue into the forseeable future % phrase "continue".
for the forseeable future           % phrase drop.
fail to successfully                % phrase "fail to" is sufficient.
Clearly,                            % syntax starting a sentence with clearly confuses me.
in different continents             % phrase ON different continents, IN different countries
(we|to) handle                      % phrase use a more specific verb like address, treat, solve
handling                            % phrase use a more specific verb like addressing, treating, solving, mitigating (unless handling errors or exceptions)
For the purposes of                 % phrase "For"
We observe that                     % phrase drop.
some degree of                      % phrase "some"
in the problem of                   % phrase (contributed by rap)
conclude several things             % phrase make (draw) several conclusions
extra bonus                         % phrase "bonus"
added bonus                         % phrase "bonus"
it is important to emphasize that   % phrase use diction to emphasize.
it is possible that                 % phrase "x may y"
caused due to                       % phrase "caused by"
recent work by                      % phrase could maybe be dropped, as the cite will include the date.
identify the location of            % phrase "find"
that go across                      % phrase "that cross"
ideally, we would like              % phrase "we would like"
enabling the ability to             % phrase "supporting" or "allowing" or "permitting"
absolutely essential                % phrase essential is.
we essentially do                   % phrase essentially is a poor adverb.  "The essence of our algorithm is a..."
Essentially,                        % phrase maybe "In essence," but could also be removed.
In this section (we|I)              % phrase "In this section, we", or "In this section, I"
essentially all                     % phrase "most"
past experience                     % phrase "experience" http://www.cmu.edu/styleguide/trickywords.html
particulary difficult primarily     % phrase simplify
intuition about why                 % phrase "intuition as to why"
Recall from above                   % phrase "recall"
Further, (I|we) will also           % phrase drop further or also
respectively                        % phrase unneeded.
in terms of                         % phrase don't need this.
the extent to which                 % phrase "how much"
make sure                           % phrase "ensure"
make up                             % phrase "constitute" "compose"
make use of                         % phrase "use"
make a decision                     % phrase "decide"
make a guess                        % phrase "guess"
since that time                     % phrase "since then"
choices to make                     % phrase "choices"
certain limitations                 % phrase what does 'certain' add to limitations?
will [a-z]* in the future           % phrase "will"
business entities                   % phrase "businesses"
rely primarily on                   % phrase "primarily" weakens "rely".  perhaps just "use" would be simpler.
has the potential to                % phrase can
have not yet developed              % phrase "have yet to develop"
to be effective,                    % phrase probably redundant.
provide information about           % phrase "tell how" "reveal" "expose" "disclose"
are different,                      % phrase "differ"
have already been                   % phrase "have been"? "were"?
as appropriate                      % phrase not needed?
only rarely                         % phrase "rarely" is probably enough.
is effective at                     % phrase "can"
foremost among them is              % phrase "foremost is" would be shorter.
those that have no                  % phrase those without
that have no                        % phrase "without"?
a variety of diverse                % phrase redundant
be highly valuable in               % phrase simplify.
the overall goal                    % phrase 'the goal'
sometimes an? [a-z]+ will           % phrase an x may
this is perhaps because             % phrase this may be because
adding an additional                % phrase redundant
IP protocol                         % phrase redundant
works well                          % phrase be more specific.
something                           % phrase could eliminate.
to keep from                        % phrase "to avoid"
[\.,] since (!then)                 % phrase probably you mean "because" unless you're talking about time. -- "has since" is okay.
performance characteristics         % phrase rare that characteristics adds.
takes into account                  % phrase considers
specify particular                  % phrase if specifying, particular should be redundant.
prototype implementation            % phrase "implementation" is redundant.
given a particular                  % phrase "given a" is probably enough
described in detail (in|below)      % phrase use "detailed"
relatively more                     % phrase more is already relative.
focus primarily on                  % phrase bad metaphor: subject of focus is singular.
primary focus                       % phrase bad metaphor: subject of focus is singular.
relatively more                     % phrase more is already relative.
gives [a-z]+ [a-z]+ information about % phrase use "tells" x
gives [a-z]+ information about      % phrase use "tells" x
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
have an effect on                   % phrase "affect"
an important question to ask is     % phrase just ask it.
an interesting thing                % phrase avoid saying something is interesting.  if you have to say it, it isn't.
checks to see if                    % phrase "checks" or "determines"
we can see                          % phrase "we can see" isn't formal enough.
still remain                        % phrase "remain".
change over time                    % phrase "change"
turn into                           % phrase "become"
looking back in retrospect          % phrase pick.
ensures that there will be no       % phrase "prevents"
does have                           % phrase "has"
first step toward this              % phrase "toward this" can probably be dropped.
can potentially be                  % phrase "might be", or just "can be"
obviates the need for               % phrase just obviates x, not obviates the need for x.
it is indeed                        % phrase "it is", though still passive.
planning in advance                 % phrase when else might you plan?
a lot of                            % phrase "many"
keep in mind                        % phrase "consider" (or drop)
it is clear that                    % phrase if clear, you don't have to say it.
especially true                     % phrase true is an absolute, can't be especially true.
making it increasingly difficult    % phrase preventing, discouraging, impeding, blocking, slowing...
is potentially                      % phrase "may be"
have been [a-z]* in the past        % phrase 'in the past' is redundant with tense.
amount of time  % phrase "duration"
should ideally % phrase "should"
are of great benefit to % phrase "help" or "aid"
are of benefit to % phrase "help" or "aid" or "promote"
important here % phrase consider "relevant"
while at the same time % phrase "while" is enough.
are able to % phrase can
subvert the proper operation of % phrase subvert
speed slow % phrase speed is probably redundant.
of size no smaller than % phrase "of size" is probably redundant
of size no larger than % phrase "of size" is probably redundant
of size smaller than % phrase "of size" is probably redundant
of size larger than % phrase "of size" is probably redundant
might potentially % phrase "might"
in the context of % phrase "in" avoid, if possible.
increase the amount of % phrase probably just increase.
show the difference between % phrase compare
in addition, we also % phrase pick.
overhead efficiency % phrase huh?
have an effect on % phrase "affect"
have a signficant effect on %  phrase "affect"
we find % phrase can usually be removed
this suggests % phrase remove or make more precise
effective for providing	   	 % phrase remove
we performed a                   % phrase just use the verb directly
we perform a                     % phrase just use the verb directly
were able to                     % phrase could
are able to                      % phrase can


==> sections/10-previous-intro.tex <==
\ahintext{Previous intro below:}
Navigating and analyzing large datasets poses significant challenges in today's data-driven world.
%
Probabilistic topic models (\lda{}, \citealt{blei2003lda}) represent documents as mixtures of topics, with topics defined as probabilistic distributions over words. Neural topic models integrate pre-trained transformer representations into an \lda{}-like process (\ctm{}, \citealt{bianchi2020pre}) or use them in combination with clustering techniques (\bertopic{}, \citealt{bertopicMark}). 
%
These models characterize topics as list of most probable keywords. %low-level
%
While users can analyze these low-level topics to derive high-level concepts that are more interpretable and descriptive to humans~\cite{Asmussen2019SmartLR}, these methods do not always produce interpretable topics useful for end-users analysis~\cite{hoyle2021automated}. %and valuable

% For example, in a scenario where a school principle wants to evaluate the good and bad teaching practices for teaching math given a set of teacher-student conversation documents for the school year, a classical topic model generates topics \textit{`round', `card', `win', `game', `winner'}\dots based on word frequency.
For example, if a social scientist aims to explore the common characteristics of land and wildlife in government policies, a classical topic model might generate a relevant topic such as \textit{`land', `forest', `area', `wilderness', `management'}\dots based on word frequency.
%
% Yet, these keywords are mathematical terms discussed most frequently in classrooms, which lack informativeness to help researchers in the given scenario to analyze and identify abstract topics to answer their question.
Yet, the effectiveness of keyword-based topic representation in real tasks, compared to discrete descriptions that synthesize these keywords into more interpretable concepts, remains unclear.
%compared to discrete descriptions from prompt-based topic models remain unclear. 

\jbgcomment{Below paragraphs don't belong here, move to next section}

\mm{}s such as GPT~\cite{openai2024gpt4,touvron2023llama} have gained popularity for inducing topics for content analysis.
%
\topicgpt{}~\cite{pham2024topicgpt} iteratively prompts GPT-4 with random sampled documents to generate high level concepts and assigns topics to all documents. 
%
\lloom{}~\cite{lam2024concept} uses \mm{}s to extract summaries from individual documents, and synthesize them to produce high-level and human readable topics. 
%
These prompt-based topic models are reported to produce topics that are more aligned with gold labels and more descriptive~\cite{lam2024concept}.
%
However, they come with certain drawbacks. %there are downsides of current prompt-based topic models. 
%
%Prompt-based topic models require many steps 
One key issue is that they require multiple rounds of prompting across many documents, which can become costly as the data size scales.
%
%In addition, there still lacks work evaluating how much can 
Additionally, there is still a lack of research evaluating how effectively prompt-based topic modeling help users build a mental model and analyze the dataset from scratch, which is the ultimate goal of topic modeling. This raises an import questions: are prompt-based approximations of topic models truly more useful for data analysts?
%leading to the question: are newer topic models more useful for data analysts?


With the increased interactive capabilities of \mm{}s, we also include \bass{}, an interactive interface that prompts \mm{}s to generate summary and topics for individual documents. Users can then edit the topics as feedback for the \mm{}, guiding it to generate more meaningful topics aligned with their intent. 
%
We use \abr{tenor}~\cite{alto, li-etal-2024-improving} to direct users' attention to the most relevant documents one at a time, reducing the number of topics they need to read.
%the individual documents that are the most beneficial to the users sequentially and reduce the number of documents humans need to read.
%

% \jbgcomment{Run style checking script, "conduct" should always be replaced with real verb}


%We measure how much the users learn with their change of confidence after using the tool and having experts to evaluate their responses.

% We propose \bass{}, an approach that combines prompt-based topic induction (fully automated) and active learning (fully manual) with human-in-the-loop to derive high-level topics from unstructured text data.
% %
% Our approach 1) iteratively selects the most informative document is based on previously induced topics through active learning 2) An \mm{} analyzes the document, its dominant topic keywords, and similar snippets from the same topic, then generates high-level concepts with descriptions and explanations; 3) A classifier--\textit{`bandit'}--, trained with user feedback, assesses the confidence of an \mm{}-induced topic. Users collaborate with \mm{}s in inducing topics, where \mm{}s generate concepts and users edit/approve them when the \textit{bandit} model detects low confidence.


% We create a single interface for \bass{} for users to conduct content analysis. \bass{} shows advantages compared to current topic model methods:
% \begin{enumerate}
%     \item \bass{} reduces the number of prompts needed for topic induction and can scale up for large text data.
%     \item \bass{} retain good quality concepts compared to fully prompt-based methods by traversing through a fraction of the most informative documents.
%     \item The \textit{bandit} model asks human assistance on low-confident induced topic and improves faithfulness of \mm{} outputs.
%     \item \bass{} generates high-level and more interpretable topics than classical topic models. It reduces users' mental effort for content analysis and help users capture meaningful concepts for data analysis and exploration.
% \end{enumerate}


%
% Additionally, \mm{}s can generate undesirable outputs that deviate from given contents and context~\cite{xu2024hallucination}, making the outputs unsatisfiable to users due to the lack of human intervention and evaluation during topic generation.
%
% Additionally, current prompt-based topic model evaluations focus on datasets that have generic one-word gold labels that often appear in the traditional topic model keyword lists such as \textit{Health, Defense, etc}~\cite{pham2024topicgpt}, which is okay and easy to prompt a \mm{} without human validation in the generation process. When it comes to datasets with more complex research goals, fully relying on \mm{} generated topics without human intervention or feedback can lead to undesirable outputs that deviate from given contents and context~\cite{xu2024hallucination}, making the outputs unsatisfiable to users due to the lack of human intervention and evaluation during topic generation. We focus on two datasets, where one dataset has generic labels for easy of comparison with existing work, another dataset is a teacher and student conversation in a math classroom to access teaching practices associated with overall high-quality math teaching~\cite{xu2024promises} (\abr{ncte}). \abr{ncte} has gold expert defined high-level concepts that require full understanding of education, teaching, and the dataset to derive, not just based on word frequencies-- Mathematical Language: captures how fluent teacher and students use mathematical language in a classroom. We have experts to evaluate outputs from \bass{}, other prompt-based methods, and \lda{} against the gold defined high-level concepts. 

% \citet{alto, li-etal-2024-improving} showed that combining topic modeling with active learning can reduce the number of documents required for topic induction. While topic models offer users a global overview of the entire dataset, active learning directs users' attention to the most informative text snippets. 

%These traditional topic models characterize topics as lists of most probable keywords (e.g., \textit{`health'}, \textit{`insurance'}\dots) and are popular for extracting low-level keywords from unstructured texts. 
%
%Users use the low-level topics to analyze text data and synthesize into high-level concepts that are more interpretable and descriptive to humans~\cite{Asmussen2019SmartLR}.
%
%However, traditional topic models can produce incoherent and less interpretable topics that are less useful for users to conduct data analysis~\cite{hoyle2021automated}.

%%%
% {\color{blue} In today's data-driven world, navigating and analyzing large datasets poses significant challenges. Bayesian-based topic models (\lda{}, \citealt{blei2003lda}) represent documents as mixtures of topics, with topics defined as probabilistic distributions over words under a Bag-of-Words (BoW) assumption. Recent neural approaches integrate pre-trained Transformer-based representations into an LDA-like process (\ctm{}, \citealt{bianchi2020pre}) or employ them in combination with clustering techniques (\bertopic{}, \citealt{bertopicMark}) . These methods --here classical topic models-- typically characterize topics as lists of words sorted by probability within the theme (e.g., \textit{`health'}, \textit{`insurance'}\dots), making them popular tools for extracting concepts from large collections of unstructured texts. However, despite their popularity and utility, they often produce topics that are less interpretable and less valuable to end-users~\cite{hoyle2021automated}.} 

% For example, the typical outputs of a topic from a classical topic model are \textit{`trade', `country', `export', `foreign', `cuba'}\dots, which requires users to analyze related documents and synthesize the topic keywords into abstract and concrete concepts that are easier for human to interpret-- \textit{"Trade: the exchange of goods or services with individuals, organizations, or foreign countries"}. 
% %
% Topic synthesis requires significant user efforts when the data size and number of topics get large. Nonetheless, classical topic models face the challenge of producing overly generic or specific keywords that are not useful to users~\cite{hoyle2021automated, li-etal-2024-improving}. 


%
% Users then face the task of manually analyzing these documents to synthesize the keywords into more interpretable concepts-- \textit{``Trade: the exchange of goods or services with individuals, organizations, or foreign countries''}. 
% Users then face the task of manually analyzing the  
%
% This manual process can be very time-consuming, especially when dealing with large datasets or high number of topics, and is made more challenging by the lack of guiding pointers to relevant documents.
%However, this process requires significant user efforts when dealing with large datasets or a high number of topics, especially when users have to manually pick documents to analyze without pointers.

% {\color{blue} For example, classical topic models might generate keywords like \textit{`trade', `country', `export', `foreign', `cuba'}\dots to identify a topic under which a set of documents are active. Yet, these keywords can sometimes be overly generic or specific and thus not very useful to end-users~\cite{hoyle2021automated, li-etal-2024-improving}. Users then face the task of manually analyzing these documents to synthesize the keywords into concepts that are more easily interpretable-- \textit{``Trade: the exchange of goods or services with individuals, organizations, or foreign countries''}. However, this process requires significant user effort, particularly when dealing with large datasets or a high number of topics.}

% \mm{}s such as GPT, Claude, LLaMA, Mistral~\cite{openai2024gpt4,touvron2023llama,jiang2023mistral} recently gain popularity for summarizing and inducing abstract concepts and topics from unstructured text data for their instruction following and text understanding ability.\footnote{\url{https://claude.ai}} 
% %
% \citet{pham2024topicgpt, reuter2024gptopic} iteratively prompt a \mm{} with random sampled documents to generate high level concepts, followed with merging similar topics, and assigning refined topic concepts to individual documents. \citet{lam2024concept} uses \mm{}s to extract key sentences from individual documents, summarize documents, then generate and synthesize concepts and rationales from summarized contents. 
% %
% These prompt-based concept induction techniques produce more high-level and human-interpretable concepts with descriptions than classical topic model keywords. 

% \mm{}s such as GPT, Claude, LLaMA, Mistral~\cite{openai2024gpt4,touvron2023llama,jiang2023mistral} have gained popularity for inducing topics from unstructured text data.\footnote{\url{https://claude.ai}} 
% %
% \citet{pham2024topicgpt} iteratively prompts GPT-4 with random sampled documents to generate high level concepts, followed with merging similar topics with GPT-3.5-turbo, and assigning refined topic to individual documents. 
% %
% \citet{reuter2024gptopic} introduces a method akin to BERTopic but allowing for a fixed number of topics and using agglomerative clustering, defining topics through titles, descriptions, assigned documents, and document embeddings, with RAG enabling dynamic interactions via a chat interface. 
% %
% \citet{lam2024concept} uses \mm{}s to extract key sentences from individual documents, summarize documents, then generate and synthesize concepts and rationales from summarized contents. 
% %
% Prompt-based techniques generate more human-understandable and descriptive concepts than traditional topic models.


% {\color{blue}
% \mm{}s such as GPT, Claude, LLaMA, Mistral~\cite{openai2024gpt4,touvron2023llama,jiang2023mistral} have recently gained popularity for inducing concepts or topics from unstructured text data.\footnote{\url{https://claude.ai}} 
% %
% \citet{pham2024topicgpt} iteratively prompt a \mm{} with random sampled documents to generate high level concepts, followed with merging similar topics, and assigning refined topic concepts to individual documents. \citet{reuter2024gptopic} introduce a method akin to BERTopic but allowing for a fixed number of topics and employing agglomerative clustering, defining topics through titles, descriptions, assigned documents, and document embeddings, with RAG enabling dynamic interactions via a chat interface. \citet{lam2024concept} uses \mm{}s to extract key sentences from individual documents, summarize documents, then generate and synthesize concepts and rationales from summarized contents. 
% %
% These prompt-based techniques generate more human-understandable concepts compared to traditional topic models.
% }

%
% However, current prompt-based topic modeling methods often face challenges at scaling up the data size that requires prompting the \mm{}s many times, which can be expensive in money and time. Additionally, \mm{}s can hallucinate and generate concepts or topics that deviate from given contents~\cite{xu2024hallucination}, and existing \mm{}-based approaches lack human supervision and evaluation of \mm{} outputs during the topic generation phase; the evaluations mainly rely on comparing generated topics with the \textit{'gold standard'} without using related documents to support the quality and validity of the generated topics. 
% %
% Humans want some trust in the \mm{} but not all to help them analyze unstructured data, and the interaction between \mm{}s and humans with thresholds becomes necessary, which human only supervise \mm{} outputs when necessary.

% {\color{blue} However, current prompt-based topic modeling methods face challenges in scaling up data size, requiring multiple prompts that can be costly in terms of both money and time. Additionally, \mm{}s can generate hallucinated concepts that deviate from given contents~\cite{xu2024hallucination}, making their output untrustworthy to end-users due to the lack of human supervision and evaluation during topic generation-- SOTA evaluations mainly rely on comparing generated topics with \textit{`gold standard'} labels without using related documents to support the quality and validity of the generated topics.  To build trust, it's crucial to establish thresholds for human-\mm{} interaction. This way, humans can supervise \mm{} outputs selectively, ensuring reliable analysis of unstructured data.
% }



% mainly rely on comparing generated topics with \textit{`gold standard'} labels without using related documents to support the quality and validity of the generated topics. To build trust, it's crucial to establish thresholds for human-\mm{} interaction, where humans can supervise \mm{} outputs selectively, ensuring reliable analysis of unstructured data.


%
% Then users can induce topics based on their interaction with topic model keywords, document clusters, and the selected document throughout the topic induction process.

% We leverage prompt-based topic induction approaches (fully automated with no human assistance) and active learning approach (fully manual) and propose \bass{}: a topic induction approach that integrates classical topic models, \mm{}s, and human to induce and learn high-level/abstract concepts from unstructured text data. 
% %
% \bass{} uses active learning to iteratively pick the most informative document based on previous induced topics. 
% %
% A \mm{} analyzes the document, its dominant topic keywords, and similar document snippets from the same topic, then generates high-level concepts with description and explanation.
% %
% Specifically, we introduce \textit{`bandit'}, a classifier trained with user feedback that checks the confidence of a \mm{} induced topic.
% %
% We have users collaborating with \mm{}s to induce topics, which \mm{}s are responsible for concept generation and users are responsible for editing/approving \mm{}-induced concepts when \textit{bandit} model detects low confidence. 

% {\color{blue} We propose \bass{}, an approach that combines prompt-based topic induction (fully automated) and active learning (fully manual) within a user-in-the-loop methodology to derive high-level concepts from unstructured text data. Our approach is three-fold: 1)  The most informative document is iteratively selected based on previously induced topics through active learning; 2) An \mm{} analyzes the document, its dominant topic keywords, and similar snippets from the same topic, then generates high-level concepts with descriptions and explanations; 3) A classifier--\textit{`bandit'}--, trained with user feedback, assesses the confidence of an \mm{}-induced topic. Users collaborate with \mm{}s in inducing topics, where \mm{}s generate concepts and users edit/approve them when the \textit{bandit} model detects low confidence.
% }

% We propose \bass{}, an approach that combines prompt-based topic induction (fully automated) and active learning (fully manual) with human-in-the-loop to derive high-level topics from unstructured text data.
% %
% Our approach 1) iteratively selects the most informative document is based on previously induced topics through active learning 2) An \mm{} analyzes the document, its dominant topic keywords, and similar snippets from the same topic, then generates high-level concepts with descriptions and explanations; 3) A classifier--\textit{`bandit'}--, trained with user feedback, assesses the confidence of an \mm{}-induced topic. Users collaborate with \mm{}s in inducing topics, where \mm{}s generate concepts and users edit/approve them when the \textit{bandit} model detects low confidence.


% We create a single interface for \bass{} for users to conduct content analysis. \bass{} shows advantages compared to current topic model methods:
% \begin{enumerate}
%     \item \bass{} reduces the number of prompts needed for topic induction and can scale up for large text data.
%     \item \bass{} retain good quality concepts compared to fully prompt-based methods by traversing through a fraction of the most informative documents.
%     \item The \textit{bandit} model asks human assistance on low-confident induced topic and improves faithfulness of \mm{} outputs.
%     \item \bass{} generates high-level and more interpretable topics than classical topic models. It reduces users' mental effort for content analysis and help users capture meaningful concepts for data analysis and exploration.
% \end{enumerate}

%{\color{blue} 
%We have integrated \bass{} within a single interface so users can conduct content analysis. Altogether, \bass{} offers several advantages over current topic modeling methods:
%\begin{itemize}
%    \item \bass{} reduces the number of prompts needed for topic induction and can scale up for large datasets.
%    \item Compared to fully prompt-based methods, \bass{} maintains high-quality concepts by analyzing only a fraction of the most informative documents.
%    \item The inclusion of the \textit{bandit} model prompts human assistance for low-confidence-induced topics, enhancing the faithfulness of \mm{} outputs.
%    \item \bass{} generates high-level and more interpretable topics than classical topic models, reducing users' cognitive load for content analysis and enabling them to capture meaningful concepts for data exploration and analysis.
%\end{itemize}}


% These topic keywords overlooks the abstract concepts that can be derived by looking at the document clusters and keywords, which are more useful for human to conduct content analysis to understand what is in the documents sets, such as \textit{`Trade: mentions the exchange of goods with other parties or foreign countries'}.


% They are popular for various applications in various fields, from text applications such as data exploration, content analysis to dimensionality reduction for classification. However, the power of topic models can be limited by their unsupervised nature, where the final clusters are simply based on word frequency distributions or pre-trained word embedding similarities. 

% where there is no human intervention or control of the generated topics; the final clusters are simply based on word frequency distributions or pre-trained word embedding similarities. On the other hand, although supervised topic models and labeled topic models can form topics based on pre-labeled human input labels, but they require users to first iteratively go through the documents and start making label categories from scratch, which can be labor-intensive and time-consuming. 

% Topics convey important information for data analysis and exploration, where users get a global sense of various topics in the documents, and analyzing related documents within different topics. The process of exploratory data analysis (\abr{eda}) can be started from the topics and analyze the documents, or from analyzing the documents to forming the topics depending on the purpose of the users. With the help of powerful large language models, we list out several contributions:

% \begin{itemize}
%     \item A topic model technique that forms topics by actively selecting documents from a set of documents, with large language models generating a generalizable topic based the actual contents of the documents rather than pure word distributions
%     \item We use active learning to greatly reduce the number of documents needed for prompt the \abr{llm} to generate topics
%     % \item Human supervised topic formation process: users can interrupt the process of topic formation by the \abr{llm} to supervise the quality of the new-formed topics
%     \item Evaluation: we propose new automatic evaluations to evaluate between classical topic models and \abr{llm} topic model
%     \item We conduct human ratings for the output topics with most associated formed
%     \item Our propose topic model combines the advantage of both classical topic models (access to document topic distribution that represent the lower level features of the documents) and topic models using \mm{}s (have a specific description for the topics instead of a list of keywords, where the topics are generated based on the actual contents from the documents.)
% \end{itemize}


==> sections/70-Evaluation.tex <==
% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[trim={0cm 0cm 0cm 0cm}, clip, width=\textwidth]{figures/bills_boxplot.pdf}
%         \caption{Bills}
%         \label{fig:boxplot_bills}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.45\textwidth}
%         \centering
%         \includegraphics[trim={0cm 0cm 0cm 0cm}, clip, width=\textwidth]{figures/news_boxplot.pdf}
%         \caption{News}
%         \label{fig:boxplot_news}
%     \end{subfigure}
%     \caption{..}
%     \label{fig:boxplots}
% \end{figure*}

% \subsection{IDEA 1: Test for Specificity}
% Train/Set set evaluation.:
% \begin{itemize}
%     \item Select a fixed set of documents from the test set, and some documents from the train set, use it as the validation set.
%     \item Within each group, show users document sequentially. For each document, show the user the top 20-30 generated topics sorted by highest cosine similarity or relevance to the document. Let them match the topic to the document. For traditional topic models, show the users the topic keyword lists and let them match the topic keywords to documents.
%     \item At the end, calculate the inter-annotator agreement within each group. Or the coverage rate/accuracy, time/speed, mental challenge rating...
%     \item The train/test set split tests for generalization, interpretability of topics, quality of topics. Also tests the generated topics are not overly specific.
% \end{itemize}

% \subsection{IDEA 2: Test for too Generic}
% Train/Set set evaluation.:
% \begin{itemize}
%     \item Make the heldout test set such that some generic gold topic categories are not in the train set. For example, \textit{Health} is only in test set but not train set.
%     \item Within each group, show the users documents sequentially with top 20-30 relevant topics for each document. Ask the users if any can be a choice. If not, select none.
%     \item At the end, calculate the nones in each group. The more nones are in each group, we have better control on the generality of the topics.
% \end{itemize}

% \subsection{IDEA 2: Test for too Generic}
% Train/Set set evaluation.:
% \begin{itemize}
%     \item Select a fixed set of documents from the test set, and some documents from the train set, use it as the validation set.
%     \item Within each group, show users document sequentially. For each document, show the users the top 20-30 most relevant topics and add a distractor (can be a very generic topic: living things, organisms). Calculate the times the users can successfully pick the distractors for each group.
%     \item The generic distractors measures the generated topics or keywords are overly generic.
% \end{itemize}


% {\color{red}Formula Calculation to balance between specifity and generality:

% Use the F1 Precision and Recall formula.}

% NOTES: we let the users who have been through the \bass{} process to do follow-up test evaluation for each of the group. I suspect the users are more efficient and faster for the \bass{} topics. Then hire more users other than \bass{} users to do the same test set evaluation and check the results. This way we can measure users who have been through the content analysis process can better use and learn the generated topics than using topics from fully automated methods without going through the process. 

% %
% For users who have not been through the process but use the \bass{} topics to match test set documents, if the matching rates are similar to TopicGPT, better than LDA, then we can conclude that \bass{} retain high quality topics compared to TopicGPT even though it only traverses through only a fraction of the documents. We can also conclude that the generalization and interpretability of \bass{} topics from one user to a different user. 


% Once we have the above two conclusions, we can synthesize and say that 

% 1. users been through \bass{} can generate good quality labels that are more descriptive and can be understood by other users; 

% 2. users been through the \bass{} process learns more from the concepts, contents of the documents, and topics so they can match the labels to test documents more efficiently and with less effort than handing them a list of topic keywords or a list of topics fully generated by \mm{}s.  


% \subsection{IDEA 4: Coverage Rate between golds}
% \begin{itemize}
%     \item For each generated topic or topic keywords, let an LLM find whether the generated topic has a semantic similar/equivalent gold label from the gold label list
%     \item The higher the coverage rate, the better
% \end{itemize}

% \subsection{IDEA 5: Clustering evaluation}
% Train/Set set evaluation.:
% \begin{itemize}
%     \item Select a fixed set of documents from the test set, and some documents from the train set, use it as the validation set.
%     \item For each document, show the user the most relevant top 10 topics from each group (LDA, TopicGPT, CTM...). Let the user pick the most descriptive group. Or add a distractor option, let the user pick the distractor.
% \end{itemize}




% \subsection{IDEA 4: Clustering evaluation}
% Active learning with \mm{} is the only method that can show an increasing of clustering qualities among all the methods. We show the clustering evaluations for all the methods, and the evolution of the metrics for \bass{}.

% % \subsection{Advantages}
% % Our proposed method is the transferring and adjustment of classical topic models to \mm{}-based topic models. We retain the initial low-level features for classical topic models in the first place, but use that as an advantage to cluster similar documents that have similar labels generated by the \mm{}. Our final output of the topic model is a classifier, with tf-idf document embedding, and a document pairwise matri, and a assigned topic for each document. In comparison, TopicGPT only has an assigned topic for each document but no access to the pairwise matrix. 

% % \subsection{Automatic Evaluation Ideas}
% % \begin{itemize}
% %     \item Document matrix pairwise score?
% %     \item Balance of the topics?
% %     \item Alignment with a reference graph. Since we do not have access to a ground-truth reference graph (it would only be available if we were to use synthetic data, but we cannot use synthetic data when LLMs are involved), we replace it with an approximation based on the document metadata \cite{vazquez2022validation}. 
% % \end{itemize}

% \subsection{Human Validation of Topics}
% \begin{itemize}
%     \item Select the most related document for each topic, let users justify whether a label is better or a list of topic keywords is better
%     \item Select a document, show the user the topic keywords, and \mm{} labels and see which one is better. Related the documents with topics.
% \end{itemize}

% \subsection{Standard Evaluation}
% Mainly Bills dataset
% Purity, RandIndex, NMI.

% Human evaluation: 
% For each topic model method, we show the users all the gold labels, and the topic model topics. Ask them whether the topic model topics match any of the gold topics. Calculate the coverage rate of the topics. We assume the rate is high for all prompt-based methods.


% \paragraph{IDEA 5: }
% Give users a set of documents, and for each document the labels generated by each model (e.g., Lloom, Tenor, BASS, gold label as baseline) + topic keywords. People evaluating this is not the same that generated them.

% \subsection{Expert High-Level Evaluation} 
% Mainly on the \ncte{} dataset. The datasets have high-level expert defined concepts that can be used to answer research questions. We ask non-expert users to use each of the topic model method to generate descriptive labels/concepts that describe the open research question \textit{What high-inference teaching practices (i.e., MQI variables) are associated with overall high-quality math teaching?} in the dataset. We ask education study experts who have similar backgrounds and familiarity in the dataset to evaluate how closely the non expert written topics align with the gold topics; additional new insights grounded from the dataset and the topics are rewarded and not penalized, but for those not from the dataset or the topics (most likely daily common sense or google search) will be panalized.

==> sections/80-related.tex <==
\jbgcomment{I wouldn't talk about ITM here, that can go into related work.  Cite Tenor / alto in introducing bass}

Interactive topic models~\cite{Hu:Boyd-Graber:Satinoff-2011, ITM-1} allow users to iteratively interact with a topic model interface to refine topics for aiding content analysis.
%
\citet{Hu:Boyd-Graber:Satinoff-2011} adopts user constraints to selectively remove or add elements in the state of a Markov Chain used for inference to generate more interpretable and user-favored topics than unsupervised topic models. 
%
~\citet{alto, li-etal-2024-improving} propose an active learning approach that combines latent topic features and user-provided labels to generate human-formulated topics while minimizing manual labeling effort.
% 
Current interactive topic models rely heavily on human effort to refine and annotate generated topics for data analysis. 
%
We use an \mm{} in interactive topic modeling to reduce manual effort. 
%
This approach leverages \mm{}s to generate topic suggestions under user supervision, minimizing the need for complete manual creation while maintaining human control of the topics over the process.
%
Interactive topic models gives users flexibility to define topics as they explore data.
%

==> sections/900-discussion.tex <==
%% Zongxia
% \paragraph{Qualitative Analysis}
% We examined users' comments on the tool. 


\paragraph{User response time} In table \ref{table:user_response_time}, we present the average and median labeling times in seconds per document for users in each group. The NA group exhibits the shortest duration, while the NONE group takes the longest. Participants spend more time labeling without the aid of topic model keywords and highlights. While neural topic models can sometimes produce overly specific or nonsensical keywords beyond the top \(N\) (where \(N\) is dataset-dependent)~\cite{put citation}, this does not seem to hinder users' labeling experience, likely because their judgments are based on the top keywords. Additionally, highlights above a 0.05 threshold for documents in LDA, sLDA, CTM could also influence the labeling speed. Furthermore, based on automatic evaluation metrics and table \ref{table:no_topic_feature_metrics}, classical LDA does not display a significant advantage over NTM in a human-in-the-loop application, both on accelerating the labeling process and enhancing label quality.


\begin{table}[ht]
\centering
\begin{tabular}{l c c}
\hline
 & Mean & Median \\
\hline
\hline
NONE  & 30.18 & 18.0\\
\hline
LDA  & 24.16 & 15.5\\
\hline
sLDA & 22.86 & 16.0\\
\hline
CTM & 21.19 & 11.0\\ % Ensure this notation is intentional
\hline
\end{tabular}

\caption{Mean and median time participants spent labeling a document for each group in seconds}
\label{table:user_response_time}
\end{table}

% \paragraph{User Rating Scaling} In our post-study survey, participants rated the mental demand of the task on a scale of 1 to 7. We interpreted ratings above 4 as indicating above-average challenge, and those below 4 as signifying low challenge. In the NONE group, two-thirds (2 out of 3) found the task mentally demanding. For the sA group, 80\% (4 out of 5) considered it challenging, with half of them assigning a neutral score of 4. This suggests that continually updating sLDA, introducing new topics, and altering keywords can potentially increase the cognitive load for participants. They might need time and mental energy to adapt to these new changes. In the LDA group, 40\% (2 out of 5) found it demanding, whereas one participant felt it required no mental effort, rating it a mere 1. In the CTM group, 60\% (3 out of 5) considered the task mentally demanding. In all the groups, except LDA, the majority of the participants found the task to be mentally demanding. This could suggest that the one hour long session task inherently requires a degree of cognitive effort, while LDA might produce more sensible topic keywords that reduce user cognitive load.

% Participants were asked to rate their confidence in the labels they assigned to the documents on a scale of 1 to 7, with higher scores indicating greater confidence. We interpret scores above 4 as above-average confidence. In the LDA Group, all participants indicated a uniform sense of above-average confidence in their labeling. For the sLDA Group, while the majority rated a confident score of 6, one participant expressed a lower confidence of 3. This disparity might hint that updating models can occasionally undermine user confidence. In the NONE Group, two participants responded below-average confidence. The presence of relevant topics and keywords as cues could both guide or inadvertently influence users' decisions: while they can guide users, any deviation from the suggested keywords or topics might dent their confidence, especially if their labels don't align with these hints. More than half of the NA Group participants rated their confidence as below average. This observation is intriguing; even though automatic evaluation metrics suggest advantages for the NA group over other groups in terms of label quality and time efficiency, there appears to be a gap in user confidence. This discrepancy could lead us to question the efficacy of the NTM. Is it making users more cautious about AI tools, or are its highly specific keyword suggestions causing doubt in users when their decisions deviate?


%% Zongxia
